Adaptive Hamiltonian and Riemann Manifold Monte Carlo Samplers

In this paper we address the widely-experienced difficulty in tuning Hamiltonian-based Monte Carlo samplers. We develop an algorithm that allows for the adaptation of Hamiltonian and Riemann manifold Hamiltonian Monte Carlo samplers using Bayesian optimization that allows for infinite adaptation of the parameters of these samplers. We show that the resulting sampling algorithms are ergodic, and that the use of our adaptive algorithms makes it easy to obtain more efficient samplers, in some cases precluding the need for more complex solutions. Hamiltonian-based Monte Carlo samplers are widely known to be an excellent choice of MCMC method, and we aim with this paper to remove a key obstacle towards the more widespread use of these samplers in practice.

==> relatedWork.tex <==
\com{Might move to be part of Introduction? Shorten}

\textbf{Riemannian Manifold HMC}:RMHMC \citep{Girolami-11} provides an automated adaptation mechanism for HMC by exploiting the Riemannian geometry of the parameter space. This allows RMHMC to adapt to the local structure of the problem by adapting the mass matrix used in HMC, allowing for efficient exploration of the target density and quick convergence. Since RMHC automatically adapts its mass matrix, the stepsize $\epsilon$ is usually fixed and only the number of leapfrog steps $L$ need be adjusted. While $L$ is a single scalar and can be chosen using the rejection rate, it is desirable to have a fully automatic method for RMHMC, especially since there is no general guidance on how this should be chosen.

\textbf{No U-turn sampler}: The No U-turn sampler (NUTS) \citet{hoffman2011no} allows for automatic tuning for both HMC's parameters in which the stepsize $\epsilon$ is tuned during the burn-in phase, after which it is fixed and the number of leapfrog steps is adjusted. $\epsilon$ is chosen using an algorithm referred to a dual averaging. $L$ is chosen using a recursive algorithm in which the number of leapfrog steps $L$ is allowed to increase until the proposal trajectory taken by the sampler begins to move back towards the initial point, with the algorithm thus preventing U-turns. 

\com{Maybe something on papers on adaptive MCMC Roberts, Atchade.} 
 

